UCF: Uncovering Common Features for Generalizable Deepfake Detection

Deepfake detection remains a challenging task due to the difficulty of generalizing to new types of forgeries. This problem primarily stems from the overfitting of existing detection methods to forgery-irrelevant features and method-specific patterns. The latter has been rarely studied and not well addressed by previous works. This paper presents a novel approach to address the two types of overfitting issues by uncovering common forgery features. Specifically, we first propose a disentanglement framework that decomposes image information into three distinct components: forgery-irrelevant, method-specific forgery, and common forgery features. To ensure the decoupling of method-specific and common forgery features, a multi-task learning strategy is employed, including a multi-class classification that predicts the category of the forgery method and a binary classification that distinguishes the real from the fake. Additionally, a conditional decoder is designed to utilize forgery features as a condition along with forgery-irrelevant features to generate reconstructed images. Furthermore, a contrastive regularization technique is proposed to encourage the disentanglement of the common and specific forgery features. Ultimately, we only utilize the common forgery features for the purpose of generalizable deepfake detection. Extensive evaluations demonstrate that our framework can perform superior generalization than current state-of-the-art methods.

==> tables/comp-with-multi-task.tex <==
    \begin{table}[tb!]
      \centering
      \caption{Comparison with recent works using multi-task learning. The metric is accuracy.}
      \vspace{-5pt}
      \scalebox{0.80}{
      \begin{tabular}{c|c|cc} \toprule
        \multirow{2}*{Training Set} & \multirow{2}*{Model} &\multicolumn{2}{c}{Testing Set (Acc)} \\
        \cmidrule(lr){3-4}
        ~& ~& FS(HQ)& F2F(HQ)\\ 
        \midrule
        
        \multirow{5}*{F2F(HQ)}& 
        LAE~\cite{du2019towards}& 0.632& \cellcolor{Gray}0.909 \\
        ~& ClassNSeg~\cite{nguyen2019multi} & 0.541& \cellcolor{Gray}0.928 \\
        ~& ForensicTrans~\cite{cozzolino2018forensictransfer} & 0.726& \cellcolor{Gray}0.945 \\
        % ~& MemoryNet~\cite{fernando2019exploiting} & 0.865& \cellcolor{Gray}0.987 \\
       % ~& Face X-ray~\cite{li2019face} & 0.857& \cellcolor{Gray}0.977 \\
        ~& Ours& \textbf{0.867} & \cellcolor{Gray}\textbf{0.992} \\
         \bottomrule
      \end{tabular}}
    %   \vspace{-0.2cm} 
      \label{tab:cmp-generalization}
    \end{table}

==> tables/crossdata.tex <==
\begin{table*}
\centering
{
\begin{tabular}
\toprule
\multirow{2}*{Method}& \multicolumn{3}{c|}{DF} & \multicolumn{3}{c|}{F2F} & \multicolumn{3}{c|}{FS} & \multicolumn{3}{c|}{NT} & \multirow{2}*{Avg.}\\
\cline{2-13}
& \small{DFDC} & \small{CelebDF} & \small{DF1.0} & \small{DFDC} & \small{CelebDF} &\small{DF1.0} & \small{DFDC} & \small{CelebDF} &\small{DF1.0} & \small{DFDC} &\small{CelebDF} &\small{DF1.0}  \\ 
\midrule \midrule
Xception \cite{rossler2019faceforensics++} &0.654 &0.681 &0.617 &0.708 &0.598 &0.745 &0.708 &0.601 &0.605 &0.646 &0.625 &0.838 &0.669\\
% \hline
Face X-ray \cite{li2020face} &0.609 &0.554 &0.668 &0.633 &0.684 &0.766 &0.646 &0.697 &\textbf{0.795} &0.613 &0.703 &0.866 &0.686\\
% \hline
F3Net \cite{qian2020thinking} &0.682 &0.664 &0.658 &0.679 &0.654 &0.761 &0.679	&0.636 &0.651 &0.672 &0.689 &0.932 &0.696\\
% \hline
RFM \cite{wang2021representative} &0.758 &0.723 &0.717 &0.736 &0.663 &0.732 &0.714 &0.591 &0.714 &0.726 &0.600 &0.846 &0.710\\
% \hline
SRM \cite{luo2021generalizing} &0.679 &0.650 &0.720 &0.687 &0.693 &0.775 &0.671 &0.643 &0.771 &0.656 &0.651 &\textbf{0.936} &0.711\\
% \hline
Ours &\textbf{0.772} &\textbf{0.730} &\textbf{0.742} &\textbf{0.787} &\textbf{0.781} &\textbf{0.786} &\textbf{0.742} &\textbf{0.800} &0.695 &\textbf{0.741} &\textbf{0.759} &0.889 &\textbf{0.769}\\
\bottomrule
\end{tabular}}
\vspace{0.1 cm}
\caption{Generalizability comparisons with state-of-the-art methods in the term of AUC. The best results are in bold. The first row denotes the training data, and the second row shows the corresponding test dataset. Our method performs favorably among the models compared.}
\label{tab result}
\vspace{-0.3 cm}
\end{table*}

==> tables/database.tex <==
\begin{table}[tb!]
  \centering
  \caption{Specifications of benchmark databases.}
  \vspace{-0.1cm}
  \scalebox{0.75}{
  \begin{tabular}{c|c|c} 
    \toprule
    Database & Video Scale &Manipulation Algorithm \\
    \midrule
    FF++~\cite{rossler2019faceforensics++}  & 1000 real, 4000 fake
  & DF~\cite{deepfake}, FS~\cite{faceswap}, NT~\cite{thies2019deferred}, F2F~\cite{thies2016face2face} \\
    DFD~\cite{dfd}      & {~~}363 real, 3068 fake
      & Improved DF \\
    CelebDF~\cite{li2019celeb}  & {~~}408 real, 795{~~} fake
   & Improved DF \\
    DFDC~\cite{dfdc}   & 1133 real, 4080 fake
   & Unpublished \\ 
   \bottomrule
  \end{tabular}
  }
  \label{tab:datasets}
%   \vspace{-0.2cm} 
\end{table}

% FaceForensics++ (FF++)~\cite{rossler2019faceforensics}, DeepfakeDetection (DFD)~\cite{dfd}, Deepfake Detection Challenge (DFDC)~\cite{dfdc}, and CelebDF~\cite{li2019celeb}.

% DeepFakes (DF)~\cite{deepfake}, Face2Face (F2F)~\cite{thies2016face2face}, FaceSwap (FS)~\cite{faceswap}, and NeuralTexture (NT)~\cite{thies2019deferred}.

==> tables/remain-three.tex <==
\begin{table}[tb!]
  \centering
  \caption{Generalization to unseen manipulations. We report the video-level AUC(\%) on the FF++ dataset, which consists of four manipulation methods(DF, FS, F2F, NT). We train on three methods and test on the other one method. The results of other methods are from \cite{xxx}.}
  \vspace{-5pt}
  \scalebox{0.85}{
  \begin{tabular}{c|cccc}
    \toprule 
    Method
    ~& DF & F2F & FS & NT \\ 
    \midrule
    
    Xception & {0.803}& 0.994& 0.762& 0.696 \\
    
    Face X-ray & {0.803}& 0.994& 0.762& 0.696 \\
    
    SRM & 0.758& 0.994& {0.913}& {0.858} \\
    %Cat(RGB,SRM)& 0.783& 0.994& 0.928& 0.889 \\
    \midrule
    
    Ours (Xception) & 0.819& 0.995& 0.966& 0.927 \\
    Ours (ConvNext) & 0.801& 0.995& 0.975& 0.957 \\
    \bottomrule
  \end{tabular}}
  
  \label{tab:ablation}
  \vspace{-0.2cm} 
\end{table}
    

==> tables/spe_lambda.tex <==
\begin{table}[tb!]
      \centering
      \caption{
      Testing AUC results obtained for different weights of specific loss on various datasets are shown. The best result is highlighted in bold font, while the results of the within-dataset are highlighted in gray. ``Avg." represents the average AUC for cross-datasets.
    %   The metrics are AUC, AP (Average Precision), and EER (Equal Error Rate). 
    %   For AUC and AP, the higher the better. For EER, the lower the better. 
    }
    %   \vspace{1mm}
      \scalebox{0.7}{
      \begin{tabular}{c|c|c|c|c|c|c}
        \toprule
        \multirow{2}*{Training} & \multirow{2}*{Method}
        &\multicolumn{5}{c}{Testing AUC}\\
        \cmidrule(lr){3-7}
        ~&~&
        FF++ & CelebDF & DFD & DFDC & Avg. \\
        \midrule
        
        \multirow{3}*{FF++}
        
        & $\lambda_2$=0.01
    & \cellcolor{Gray}{0.967} & 0.806 & 0.936 & 0.787 & 0.843 \\
    
    ~& $\lambda_2$=0.05
    & \cellcolor{Gray}{0.964} & \textbf{0.827} & 0.937 & 0.789 & 0.851 \\
    
    ~& $\lambda_2$=0.1
    & \cellcolor{Gray}{0.968} & 0.824 & \textbf{0.945} & \textbf{0.805} & \textbf{0.858} \\
    
    ~& $\lambda_2$=0.5
    & \cellcolor{Gray}{0.964} & 0.780 & 0.925 & 0.788 & 0.831 \\
    
    ~& $\lambda_2$=1
    & \cellcolor{Gray}{\textbf{0.969}} & 0.806 & 0.927 & 0.791 & 0.841 \\
    
    ~& $\lambda_2$=5
    & \cellcolor{Gray}{0.960} & 0.793 & 0.919 & 0.771 & 0.828 \\
    
    ~& $\lambda_2$=10
    & \cellcolor{Gray}{0.968} & 0.768 & 0.934 & 0.772 & 0.825 \\
    % \midrule

         \bottomrule
      \end{tabular}}
      \label{tab:lambda}
      \vspace{-10pt} 
    \end{table}


\vspace{5mm}

==> tables/xception.tex <==
\begin{table}[t]
  \centering
  \caption{Xception~\cite{8099678} detector experiences a significant performance drop when evaluated on unseen forgeries.}
  \scalebox{0.80}{
  \begin{tabular}{c|ccccccc}
    \toprule 
    \multirow{2}*{Training}
    &\multicolumn{7}{c}{Testing (AUC)} \\
    \cmidrule(lr){2-8}
    ~& DF& F2F& FS& NT &CDF &DFDC &DFD \\ 
    \midrule
    FF-DF  &\cellcolor{Gray}0.993	&0.736	&0.485	&0.736 &0.504 &0.597 &0.652  \\
    FF-F2F &0.803	&\cellcolor{Gray}0.994	&0.762	&0.696 &0.478 &0.521 &0.576  \\
    FF-FS  &0.664	&0.888	&\cellcolor{Gray}0.994	&0.713 &0.529 &0.503 &0.539\\
    FF-NT  &0.800	&0.813	&0.731	&\cellcolor{Gray}0.991 &0.564 &0.555 &0.596\\
    CelebDF  &0.432	&0.540	&0.564	&0.518 &\cellcolor{Gray}0.863 &0.502 &0.588\\
    DFDC  &0.543	&0.550	&0.587	&0.501 &0.591 &\cellcolor{Gray}0.935 & 0.587 \\
    DFD  &0.432	&0.540	&0.564	&0.518 &0.674 &0.563 &\cellcolor{Gray}0.902 \\
    
    \bottomrule
  \end{tabular}
  }
  
  \label{tab:xception-bad-gen}
  \vspace{-0.4cm} 
\end{table}
